Optimal Adaptive Multi-Valued Byzantine Agreement

In Byzantine Agreement (BA), $n$ parties, out of which $t$ can be Byzantine, run a distributed protocol to agree on a common valid input. Traditionally, these protocols have a linear latency and quadratic message complexity, making them impractical at a large scale. In their recent work, Constantinescu, Dufay, Paramonov, and Wattenhofer consider the actual number of byzantine parties $f \leq t$ and work toward decoupling the dependency on $n$ and $t$ in the complexity. They obtain a BA protocol with $\tilde{\mathcal{O}}(n + t\cdot f)$ message complexity and $\tilde{\mathcal{O}}(f)$ round complexity. However, their results are strictly limited to agreement on a binary value. Using the framework given by their work along with novel techniques, we extend these results for BA on an $L$-bit value. With $\kappa$ being a security parameter, and with optimal resiliency ($t < n/2$ in the synchronous setting or $t < n/3$ otherwise), we obtain: - In synchrony, a deterministic protocol with $\mathcal{O}(n\cdot (L + f \cdot \kappa ))$ bit complexity and $\mathcal{O}(f + \log n)$ round complexity. - In synchrony and partial synchrony, deterministic protocols with $\tilde{\mathcal{O}}(n \cdot \kappa + t\cdot (L + f \cdot \kappa))$ bit complexity and $\mathcal{O}(f)$ round complexity. - In asynchrony, a protocol with $\tilde{\mathcal{O}}(n \cdot \kappa + t\cdot(L + t \cdot \kappa))$ expected bit complexity and expected $\mathcal{O}(1)$ latency.

==> macros.tex <==
%----- Algorithm Environment ----------------------------------
\RequirePackage{algpseudocode}
%Header for Algorithms/Functionalities
\newcommand{\algoHead}[1]{\underline{\textbf{#1}}}
\newcommand{\algoHeadNoBold}[1]{ \underline{#1}}
\newcommand{\algoHeadExt}[2]{ \underline{\textbf{#1} #2}}
%Multiline Algo-States
\makeatletter
\algnewcommand{\ExtendedState}[1]{\State
\parbox[t]{\dimexpr\linewidth-\ALG@thistlm}{\hangindent=\algorithmicindent\strut\hangafter=3#1\strut}}
\makeatother
%Algorithms States
\algnewcommand\algorithmicinput{\textbf{Input:}}
\algnewcommand\Input{\item[\algorithmicinput]}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
%Algo Comments
\algrenewcommand{\algorithmiccomment}[1]{{\color{gray}// #1}}
%Inline ifs
\algnewcommand{\IIf}[1]{\State\algorithmicif\ #1\ \algorithmicthen}
\algnewcommand{\EndIIf}{\unskip\ \algorithmicend\ \algorithmicif}

%----- Box Environment -----------------------------------------
% v 2019.1.DT small skips
%---
 \RequirePackage{varwidth}
 \RequirePackage{color}
 \RequirePackage[most]{tcolorbox}%with most option


%----- Protocol Boxes
\newtcolorbox{titlebox}[5]{enhanced,center,colframe=black,colback=white,boxrule={#3},arc={#2},auto outer arc,%
%float,
 breakable,
 pad at break*=5pt,vfill before first,before={},after={},top=12pt,left=4pt,%
 enlarge top by=2pt,%enlarge bottom by=7pt,%
 fontupper=\small,
 title={\rule[-.3\baselineskip]{0pt}{\baselineskip}\normalsize\sffamily\bfseries #1}, varwidth boxed title*=-30pt, 
 attach boxed title to top left={yshift=-10pt,xshift=10pt}, coltitle=black,
 boxed title style={colback=white,boxrule={#5},arc={#4},auto outer arc}
}
 \newenvironment{systembox}[1]
 {\begin{titlebox}{Functionality \normalfont #1}{2.5pt}{1pt}{3.5pt}{1pt}}
 {\end{titlebox}}

 \newenvironment{protocolbox}[1]
 {\begin{titlebox}{Protocol \normalfont #1}{0.5pt}{0.5pt}{1pt}{0.75pt}}
 {\end{titlebox}}
 
  \newenvironment{simulatorbox}[1]
 {\begin{titlebox}{Simulator \normalfont #1}{0.5pt}{0.5pt}{2pt}{0.75pt}}
 {\end{titlebox}}
 
  \newenvironment{processbox}[1]
 {\begin{titlebox}{Process \normalfont #1}{0.5pt}{0.5pt}{1pt}{0.75pt}}
 {\end{titlebox}}

 \newenvironment{algobox}[1]
 {\begin{titlebox}{Algorithm \normalfont #1}{0.5pt}{0.5pt}{1pt}{0.75pt}}
 {\end{titlebox}}
 
 \newenvironment{funcbox}[1]
 {\begin{titlebox}{Function \normalfont #1}{0.5pt}{0.5pt}{1pt}{0.75pt}}
 {\end{titlebox}}

 
 \newenvironment{dianabox}[1]
 {\begin{titlebox}{\normalfont #1}{0.5pt}{0.5pt}{1pt}{0.75pt}}
 {\end{titlebox}}

 
\newcommand{\vin}{v_{in}}
